Unsupervised Discovery of Structured Acoustic Tokens with Applications to Spoken Term Detection

In this paper, we compare two paradigms for unsupervised discovery of structured acoustic tokens directly from speech corpora without any human annotation. The Multigranular Paradigm seeks to capture all available information in the corpora with multiple sets of tokens for different model granularities. The Hierarchical Paradigm attempts to jointly learn several levels of signal representations in a hierarchical structure. The two paradigms are unified within a theoretical framework in this paper. Query-by-Example Spoken Term Detection (QbE-STD) experiments on the QUESST dataset of MediaEval 2015 verifies the competitiveness of the acoustic tokens. The Enhanced Relevance Score (ERS) proposed in this work improves both paradigms for the task of QbE-STD. We also list results on the ABX evaluation task of the Zero Resource Challenge 2015 for comparison of the Paradigms.

==> section/complexity.tex <==
\section{Time Complexity and Storage Requirement}\label{sec:complexity}
%

\input{table/summary}.


We list time complexity and storage requirement for training the acoustic tokens and performing QbE-STD for a token set of granularity $(m,n)$ under the Multi-granular Paradigm and a lexicon with parameters $(u,v)$ under the Hierarchical Paradigm. 
%
We ignore the space complexity during the computation of the algorithms, but instead focus on the disk space required to store the results of the algorithms. 
%
For simplicity we assume every utterance in the spoken archive has the same length $T$, and there are a total of $U$ utterances in the archive.
%
We list the results in Table \ref{tab:summary} with the corresponding notations in Table \ref{tab:notation}.
%
Note that there is no distinction between the Multi-granular and Hierarchical Paradigm for most algorithms except for token decoding in Eq. \eqref{eq:3}.


\subsection{Complexity Analysis for Learning the Token HMMs}\label{sec:cc_training}
Starting with the raw features $X$ of an utterance, the original disk storage is 
$O(Tfr)$ where $T$ is the number of frames in the utterance, $f$ is the feature dimension, and $r$ is the number of bits required to store a scalar (a floating point).
%
The disk storage would then be 
\begin{equation}
O(TUfr) \mbox{    bits} \label{eq:sc_raw}
\end{equation}
for the entire spoken archive.
%
We wish to convert it to acoustic token sequences $W$ and the acoustic models $\theta$ as in Eqs.\eqref{eq:2}\eqref{eq:3}.
%
%We omit the discussion for the time complexity of the initialization step in Eq. \eqref{eq:1} since it is roughly close to the decoding step, and it is executed only once while Eq. \eqref{eq:2} and Eq. \eqref{eq:3} have to be iteratively executed until the model converges.

The training procedure used in Eq. \eqref{eq:2} to derive $\theta$ is the Embedded model Baum-Welch Reestimation algorithm \cite{rodriguez2003comparative} and the time complexity for each iteration is $O(5mTH+3m^2TH+mTHgf)$,
%
where $T$ is the number of time frames in the training utterance, 
%
$m$ is the number of states per token HMM, 
%
%$f$ is the feature dimension, 
%
$g$ is the number of Gaussians in each GMM, 
%
$H$ is the number of tokens in the transcription $W$. 
%
To simplify the discussion we assume the expected number of frames per state is roughly a dilation constant $d$, and since the number of states per token HMM is $m$, the number of frames per HMM is $md$.
%
Since the each token in the transcription corresponds to a HMM, we have $H=T/md$. The complexity of the training procedure is then
%
\begin{equation}
  O(T^2(5+3m+gf)/d)  \mbox{    secs} .  \label{eq:tc_training}
\end{equation}
which is independent of the number of distinct tokens $n$, because every training utterance only updates roughly $F$ or less distinct tokens.
%
Eq. \eqref{eq:tc_training} is quadratic to the length of the training utterance.
%
In our experiments we choose $g=1$, and since we use MFCC with first and second order derivatives as the feature $f=39$.
%
When we fixed $g$ and $f$, asymptotically speaking the only term remaining in Eq. \eqref{eq:tc_training} would be $O(T^2m/d)$, but in practice the last term $O(T^2gf/d)$ is going to dominate since $m$ is smaller than $gf$.


The disk space required to store the acoustic models $\theta$ depends on the number of parameters for the HMM, which can be further broken down into the HMM transition matrices, and the GMM parameters for the states.
%
We assume that the covariance matrices for the Gaussians are diagonal, so the number of parameters would be $O(mngf)$, where $n$ is the number of distinct HMMs, $m$ is the number states per HMM, $g$ is the number of Gaussians per state, and $f$ is the feature dimension.
%
We also assume that within each HMM, the only allowed state transitions are those to itself or to the next state, so the total number of transitions is $2nm$.
%
Therefore the total storage of the model is 
\begin{equation}
O(mngfr)   \mbox{    bits}, \label{eq:sc_training}
\end{equation}
where $r$ is the number of bits required to represent a scalar. 
%
Here $n$, $m$ and $g$ are tunable parameters for the HMMs while $f$ and $r$ are fixed. 

The decoding procedure used in Eq. \eqref{eq:3} to derive $W$ is the Token Passing algorithm \cite{lifchitz2006optimal} and the time complexity for each iteration is $O(NMTE)$, 
%
where $N$ is the total number of states, 
%
$M$ is the number of inbound nodes on the decoding tree at token transitions,
%
$E$ is the time required to compute the emission probability of each state.
%
Because the number of states per token HMM is $m$, and there are $n$ distinct token HMMs in the set, $N=mn$.
%
The total number of inbound tokens on the decoding tree at token transitions is simply the total number of distinct tokens in the worst case scenario.
%
For the the Multi-granular Paradigm $M=n$, because we allow all types of token transition during decoding, the worst case is actually the average case.
%
For the the Hierarchical Paradigm $M=v$, but note that only the top candidates in the vocabularies are considered at every node in real systems so this is a pessimistic estimate. 
%
Since $v$ is decided by the PAT-Tree and cannot be specified, we represent $v$ using Eq. \eqref{eq:mnuv}, so we have $v\leq n^{u/m}$.
%
Since we are using HMM-GMMs for the tokens in this work, $E=O(gf)$.
%
To sum up, the time complexity of the decoding procedure is 
\begin{equation}
  O(Tmn^2gf) \mbox{    secs},  \label{eq:tc_decoding}
\end{equation}
for the Multi-granular Paradigm, and 
\begin{equation}
  O(Tmn^{2u/m}gf) \mbox{    secs},  \label{eq:tc_decoding_hier}
\end{equation}
for the Hierarchical Paradigm,
which is linear to the length of the utterance and quadratic to the total number of distinct HMMs $n$.
%

The disk space required to store the acoustic token sequence $W$ for each utterance would be the number of tokens in such an utterance, which is $H=T/md$ as mentioned above, times the number of bits required to represent every token $\log n$.
%
%We use the previous assumption that the expected number of frames per state is roughly a constant $d$, and since the number of states per token HMM is $m$, the number of frames per HMM is $md$. 
%
%Since the each token in the transcription corresponds to a HMM, the length of the acoustic token sequence is then $T/md$. 
%
The disk storage of the decoded acoustic token of every utterance is then \begin{equation}
O(T\log(n)/md)  \mbox{    bits} , \label{eq:sc_decoding}
\end{equation}
which is still of course linear to the duration of the utterance.

To sum up, let $L$ denote the number of iterations the training and decoding procedure is executed, and $U$ the total number of utterances in the spoken archive.
%
The total time complexity for learning a acoustic token set at the granularity $(m,n)$ is the sum of the training and decoding procedure times the number of iterations $L$ and the number of utterances $U$, which is
\begin{equation}
O((T^2/d + Tmn^2)LUgf)\mbox{    secs}.  \label{eq:tc_token}
\end{equation}
The representations have been converted to an acoustic model set $\theta$ and all the acoustic tokens $W$, which consumes 
\begin{equation}
O(mngfr+TU\log(n)/md) \mbox{    bits}. \label{eq:sc_token}
\end{equation}
%
Depending on the application, either the model $\theta$ or the token sequences $W$ can be discarded, since the other can be derived using Eqs. \eqref{eq:2}, \eqref{eq:3} with an additional iteration.
%
When $n$ is large (there are a lot of acoustic tokens), decoding takes longer and it would be better to store the tokens sequences $W$; when $T$ is large (the utterances are long), training takes longer and it would be better to store the model $\theta$.


\subsection{Computation Complexity for the Spoken Term Detection} \label{sec:cc_decoding}
The time and memory complexity for the standard DTW algorithm is $O(T^2)$ where $T$ represents the length of the sequences to be matched, it can be further reduced to $O(T)$ time and memory complexity with FastDTW \cite{salvador2007toward}. 
%
However in the scenario here, we are trying to match a short query of length $T_q$ to a long spoken document of length $T_s$, and the time complexity for any DTW-based algorithm is still $O(T_qT_s)$ which is quadratic versus time.
%
The reason is all possible subsequences starting at every time frame has to be examined and it would take $O(T_s)$ to achieve that even if the time complexity for every subsequence can be reduced to $O(T_q)$.
%
This is also due to the fact that the pairwise distance between frames in the query and the document still has to be calculated.
%
For the baseline frame-based DTW approach, where the feature dimension is $f$, the time complexity is 
\begin{equation}
O(T_sT_qf) \mbox{    secs} , \label{eq:tc_fdtw}
\end{equation}
which is a function of the feature dimension. 
%

In the QbE-STD system proposed in section \ref{sec:distance}, we convert both the spoken documents and the spoken queries into token sequences. 
%
Since the acoustic tokens were derived from the spoken documents, so the former is available, we only have to convert the spoken queries into token sequences using the token HMMs.
%
The time complexity for this task is $O(Tmn^2gf)$ secs as in Eq. \eqref{eq:tc_decoding}, and the converted sequence takes up $O(T_q\log(n)/md)$ bits as in Eq/ \eqref{eq:sc_decoding}.
%
By converting an utterance to acoustic tokens of granularity $(m,n)$, the length of the utterance has been reduced to $T/md$ and at each token position only $n$ possible token candidates are possible.
%
This restriction significantly reduces the number of possible outcomes for the pairwise distances between the tokens, which can then be precomputed all at once before even knowing the query.
%
Alternatively, we can also compute them on the way and cache the distances as we perform the token distance calculation in Eq. \eqref{eq:dtw}.
%
In either case, the process of pairwise distance calculation can be considered as a simple table lookup which takes O(1), so the time complexity of token-based DTW is 
%
\begin{equation}
O(T_sT_q/m^2d^2) \mbox{    secs} , \label{eq:tc_tdtw}
\end{equation}
%
which is no longer a function of feature dimension, and the distance table takes up 
\begin{equation}
O(n^2r)   \mbox{    bits} \label{eq:sc_dist}
\end{equation}
of disk space.
%
Since we are using HMM-GMMs for our tokens, the time complexity for obtaining the pairwise distance between any two HMMs in the token set of granularity $(m,n)$ is
\begin{equation}
O(mn^2g^2f) \mbox{    secs} , \label{eq:tc_dist}
\end{equation}
with the variational approximation of the KL-divergence in Eq. \eqref{eq:soft}.
%
Since Eq. \eqref{eq:tc_dist} is not a function of size of the spoken document archive, for sufficiently large corpus the time required to compute the pairwise distance can be ignored.

To sum up, if the spoken document archive contains $U_s$ utterances, and there are $U_q$ spoken queries, then the total time complexity would be the sum of Eq. \eqref{eq:tc_token} for training the spoken archive, $U_q$ times Eq. \eqref{eq:tc_decoding} on the spoken queries, Eq. \eqref{eq:tc_dist} for the computation of the distance matrix, and Eq. \eqref{eq:tc_fdtw} for the matching of the token sequence.
%
The total time complexity is 
\begin{equation}
\begin{aligned}
O(&U_sT_s^2Lgf/d +U_sT_smn^2Lgf + U_qT_qmn^2gf \\
+ &mn^2g^2f + U_sT_sU_qT_q/m^2d^2) \mbox{    secs}, \label{eq:tc_full}
\end{aligned}
\end{equation}
%
where $m$, $n$, $g$ are the only tunable parameters. 
%
This implies it is linear to the spoken query length $T_q$ during decoding, but quadratic to the spoken document length $T_s$.
%
For large spoken archive where $U_s$ and $U_q$ is large, the time complexity is reduced to
\begin{equation}
O(U_sT_sU_qT_q/m^2d^2) \mbox{    secs}. \label{eq:tc_comp}
\end{equation}
%
The disk space required for such a system would be the sum of the space for the token models in Eq. \eqref{eq:sc_training}, the space for the token sequences for the spoken archive and spoken queries in Eq. \eqref{eq:sc_decoding}, and the distance matrix in Eq. \eqref{eq:sc_dist}.
%
The entire system takes up 
%
\begin{equation}
O(mngfr + (U_sT_s+U_qT_q)\log(n)/md + n^2r) \mbox{    bits}, \label{eq:sc_full}
\end{equation}
of disk space.
%
For a large spoken archive where $U_s$ and $U_q$ is large, the required disk space is reduced to
%Distance Complexity
\begin{equation}
O((U_sT_s+U_qT_q)\log(n)/md) \mbox{    bits}, \label{eq:sc_comp}
\end{equation}
which is independent of the size of the model, and only dependent on the choice of granularity $(m,n)$.
%
For comparison, the baseline feature-based DTW system has a time complexity of 
\begin{equation}
O(U_sT_sU_qT_qf) \mbox{    secs}, \label{eq:tc_base}
\end{equation}
while the raw features take up
\begin{equation}
 O((U_sT_s+U_qT_q)fr) \mbox{   bits}. \label{eq:sc_base}
\end{equation}
%We define $D = m/d$ being the average duration of a acoustic token in the number of frames.
%
Dividing Eq. \eqref{eq:tc_base} to Eq. \eqref{eq:tc_comp}, and Eq. \eqref{eq:sc_base} to Eq. \eqref{eq:sc_comp}, we can derive the time and disk compression ratio for the proposed system:
\begin{equation}
\begin{aligned}
\mbox{time compression ratio:} & fm^2d^2, \\
\mbox{space compression ratio:} & fmdr/\log n.
\end{aligned}
\end{equation}
%
In the time required to perform feature DTW once, it is possible to compute the distance on the same document and query using multiple token sets.
%
The Multi-granular Paradigm is not as computationally demanding as it seems.
%
We summarize the results in Table \ref{tab:notation} and \ref{tab:summary}.


%Although we assumed the duration of a state $d$ to be a fixed number of frames in our discussion, it is actually dependent of $g$, which is the number of Gaussian components in the GMM. 
%
%The larger $g$ is the more variation it would be able to model, resulting in a longer $d$.

%f*g^2 for every 2 GMM
%n^2*m*f*g^2 in total
 
%Decoding Complexity
%n^2*m*T1*g*f
 
%Matching Complexity
%T1/(dm)*T2/(dm)=T1T2/(dm)^2
 
%Distance Storage
%n^2*r

==> section/hierarchical.tex <==
\section{The Hierarchical Paradigm}\label{sec:hier_par}

The Hierarchical Paradigm automatically learns the word-like and subword-like tokens, as well as all relevant knowledge for this set of tokens such as the lexicon and N-gram language model referred to as the linguistic structure for the spoken language of the given corpus.
%
The goal is to find the parameter set $\theta=\{\theta^a,\theta^x,\theta^l\}$ for the linguistic structure, and the word-like token label sequences $W$ on the observed acoustic feature vector sequences $X$ for the corpus considered. 
%
The parameter set $\theta$ includes three parts: $\theta^a$ for acoustic HMMs of subword-like tokens, $\theta^x$ for the lexicon of word-like tokens in terms of subword-like token sequences, and $\theta^l$ for the word-like token N-gram language model.
%
This is achieved by first finding the initial label $W_0$ for the observations $X$ as in Eq. (\ref{eq:1}).
%
In each of the following iterations $i$, we then train the parameters $\theta_i=\{\theta^a_i,\theta^x_i,\theta^l_i\}$ with the label sequences $W_{i-1}$ obtained in the previous iteration as in Eq. (\ref{eq:2}) and decode the label sequences $W_{i}$ with the obtained parameters $\theta_i$ as in Eq. (\ref{eq:3}) \cite{gish2009unsupervised}. 


\begin{eqnarray}
W_0 &=& \mbox{initialization}(X).                                   \label{eq:1} \\ 
\theta_{i} &=& \arg \max_{\substack{\theta}} P(X|\theta,W_{i-1}),   \label{eq:2} \\
W_i &=& \arg \max_{\substack{W}} P(X|\theta_i ,W),             \label{eq:3}
\end{eqnarray}

Eq. (\ref{eq:2}) is the maximum likelihood training of HMMs, and the only difference here is that we train on the label sequences $W_{i-1}$ obtained in the previous iteration rather than ground truth labels. 
%
Eq. (\ref{eq:3}) is the Viterbi decoding based on the model set $\theta_i$.
%
After the initialization in Eq. (\ref{eq:1}) above, the following iterations in Eq. (\ref{eq:2}) and Eq. (\ref{eq:3}) are organized as three cascaded stages (I), (II) and (III) respectively for acoustic, linguistic and lexical optimization as shown in Fig. \ref{fig:FP}. 
%
In Fig. \ref{fig:FP}, the number of iterations for each stage are represented by $I_a$, $I_l$ and $I_x$ respectively. 
%
When the difference between $W_{i-1}$ and $W_{i}$ becomes insignificant, the process then advances to the next stage. 
%
The parameters $\theta^a_i$ are generated by EM training as in Eq. (\ref{eq:2}), while the other parameters $\theta^l_i$ or $\theta^x_i$ are generated directly from the labels $W_{i-1}$ obtained in the previous iteration.
%
However, not all of $\theta^a$, $\theta^x$, and $\theta^l$ are used in each stage. The detailed updating procedure will be explained shortly.

The basic idea behind the procedure in Fig. \ref{fig:FP} is to gradually construct and update the parameters layer after layer. 
%
This prevents the parameters from being caught in local optimal situations which often happen when too many parameters are optimized jointly at the same time.
%
First, the HMM parameters for the subword-like tokens are trained alone in stage (I), because these HMMs are the primary building blocks of the whole linguistic structure and reliable estimate for their parameters is the key. 
%
With reliable enough HMMs for subword-like tokens, we then in stage (II) use N-gram parameters for word-like tokens to better decode those word-like tokens frequently appearing together while continuously updating the HMM parameters.
%
Finally in the stage (III), we break the word-like tokens into subword-like tokens and reconstruct better word-like tokens. 
%
The number of word-like tokens in the lexicon may shrink in the iterations of the first two stages because some less frequent word-like tokens can be absorbed by other tokens, but this number can be changed significantly in the third stage.
%
The time alignment for the subword-like tokens are updated in all iterations when the labels $W_i$ are decoded.

\begin{figure}[tbh]
  \centering
    \includegraphics[width=0.45\textwidth]{figure/fourstagex.png}
     \caption{
	Simplified digram for the proposed initialization step followed by three stages of iterative optimization.}
     \label{fig:FP}
\end{figure}

\begin{figure}[tbh]
  \centering
    \includegraphics[width=0.45\textwidth]{figure/watershed.png}
     \caption{
An example dotplot for an utterance and its watershed transform.}
     \label{fig:WS}
\end{figure}

\begin{figure}[ht]
\centering
%\includegraphics[width=0.45\textwidth]{acoustic.png}
\includegraphics[width=0.45\textwidth]{figure/fourdetail.png}
\caption{Detailed diagrams for the three stages of (a)acoustic (b)linguistic and (c)lexical optimization.}
\label{fig:Pac}
\end{figure}

\subsection{Initialization}\label{ssec:init}
%Given an unlabelled speech corpus, it is not difficult for unsupervised discovery of the desired acoustic tokens from the corpus for a chosen hyperparameter set $\psi$ that determines the topology of the HMMs \cite{jansen2011towards}\cite{gish2009unsupervised}\cite{creutz2007unsupervised}.
%This can be achieved by first finding an initial label $w_0$ based on a set of assumed tokens for all observations in the corpus $\chi$ as in (\ref{eq:1})\cite{chung2013unsupervised}.
%Then in each iteration $t$ the HMM parameter set $\theta^\psi_{t}$ can be trained with the label $w_{t-1}$ obtained in the previous iteration as in (\ref{eq:2}), and the new label $w_{t}$ can be obtained by free-token decoding with the obtained parameter set $\theta^\psi_{t}$ as in (\ref{eq:3}). 
%\begin{eqnarray}
%w_{0}&=& \mbox{initialization}(\chi),                                           \label{eq:1} \\ 
%\theta^\psi_{t} &=& \arg \max_{\substack{\theta^\psi}} P(\chi|\theta^\psi,w_{t-1}),             \label{eq:2} \\
%w_{t} &=& \arg \max_{\substack{w}} P(\chi|\theta^\psi_{t} ,w).                        \label{eq:3}
%\end{eqnarray}
%The training process can be repeated with enough number of iterations until the difference between $w_{t-1}$ and $w_{t}$ becomes insignificant. This gives a converged set of acoustic token HMMs which we denote as $\Theta^\psi$.

The goal of the initialization step is to obtain the initial word-like token label sequences $W_0$ given the observation feature sequences $X$ for the given corpus.
%
%
Under noisy conditions the detected word-like boundaries can be suboptimal, but the initial labels do not have to be very precise, since they are be updated by many following iterations. 
%
Here we initialize the token labels in a top-down fashion by first breaking each utterance into word-like segments based on the discontinuities in a parameter evaluated from energy and MFCC features.
%
Note that the discontinuities were found based on energy activations, so in principle the word boundaries are detected like voice activity detection systems. \footnote{The exact MATLAB function used to generate the initial alignment can be found here https://github.com/C2Tao/zrst/blob/master/zrst/matlab/clusterDetection.m}. 
%
For each word-like segment, we further divide it into subword-like segments in the following way.
%
We perform a watershed transform on the filtered self-similarity dotplot \cite{jansen2010towards} for acoustic features of each hypothesized word-like segment.
%
Watershed transformation is able to capture the number of objects and their borders in a gray scale image \cite{couprie1997topological}.
%
So, the intersections of the diagonal entries of the dot-plot with the watershed transform object borders are taken as the boundaries between subword-like segments.
%
An example dotplot and its watershed transform including the hypothesized subword-like segment boundaries is shown in Fig. \ref{fig:WS}. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We then extract an average representative feature vector for every hypothesized subword-like segment, and perform global k-means clustering on these representative vectors obtained from the whole corpus.
%
The number of clusters (the initial number of subword-like tokens) is determined by the ratio of the within-cluster total scattering to the between-cluster total scattering.
%
A subword-like token ID is then assigned to each cluster.
%
A distinct sequence of consecutive subword-like tokens for a word-like segment then defines a word-like token, and the total number of distinct word-like tokens obtained from the corpus is the initial vocabulary size of the lexicon.
%
The corpus is thus represented by its initial labels $W_0$. 

\subsection{Stage (I):Acoustic Optimization}

% in terms of definition for word-like units.
A more complete plot for the process in stage (I) of Fig. \ref{fig:FP} is shown in Fig. \ref{fig:Pac}(a). 
%
In each iteration, the acoustic model set $\theta^a_i$ are the HMMs trained from the corpus based on $W_i$ with the ML criterion as in Eq. (\ref{eq:2}).
%
The lexicon $\theta^x_i$ is derived by collecting all word-like tokens appearing in $W_i$ with counts exceeding a threshold.
%
Free word decoding is then performed on the whole corpus $X$ based on $\theta^a_i$ and $\theta^x_i$, producing an updated label $W_{i+1}$.
%
When $W_i$ is updated to $W_{i+1}$, not only the HMM parameters of $\theta^a_i$ and HMM segmentation boundaries are updated, but the vocabulary size of $\theta^x_i$ may shrink when the counts of some word-like tokens become small enough.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Stage (II):Linguistic Optimization}
More details of stage (II) in Fig. \ref{fig:FP} is shown in Fig. \ref{fig:Pac}(b), which is very similar to the previous stage in Fig. \ref{fig:Pac}(a). 
%
The only difference is an N-gram language model $\theta^l_i$ for the word-like tokens is estimated from the label $W_i$ and is used in decoding to produce the updated labels $W_{i+1}$. 
%
The N-gram helps produce better labels $W_{i+1}$ especially for word-like tokens appearing together frequently. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Stage (III):Lexical Optimization}
We then reconstruct new word-like tokens in stage (III) in Fig. \ref{fig:FP} with details in Fig. \ref{fig:Pac}(c). 
%
This is achieved by breaking the word-like tokens in $\theta^x_{i-1}$ into subword-like tokens, and then reconstructing new word-like tokens based on $W_i$. 
%
Those segments of several consecutive subword-like tokens appearing frequent enough and with high enough right and left context variation are taken as new word-like tokens. 
%
This can be realized by constructing an efficient data structure called PAT-Tree using the labels $W_i$\cite{ong1999updateable}. 
%
In this way, the lexicon $\theta_i^x$ can be updated significantly in each iteration. 
%
With the PAT-Tree, single token words are often included into the lexicon.%
If a word-like token is not in the lexicon, it is usually represented by several smaller subword-like tokens.
%
This updated lexicon $\theta^x_i$ is then used in free-word decoding to produce the labels $W_{i+1}$. 
%
The whole process is completed when there is no significant difference between $W_i$ and $W_{i+1}$. 
%
This gives the automatically discovered linguistic structure $\theta=\{\theta^a,\theta^x,\theta^l\}$, where $\theta^l$ is trained from the final version of $W_{i+1}$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> section/multigranular.tex <==
\section{The Multigranular Paradigm}\label{sec:mult_par}

In this paradigm we consider the situation where an unknown number of levels of intrinsic acoustic representations exist in the spoken corpus.
%
Acoustic units with different lengths such as phonemes, syllables, words, and phrases have different temporal granularity.
%
Different phonetic clusters such as speaker-independent phonemes, gender-dependent phonemes, speaker-dependent phonemes have different phonetic granularity. 
%
We wish to develop a set of acoustic token HMMs for every different granularity configuration (temporal and phonetic) on the same corpus.
%
With multiple sets of granularity configurations, the system would have multiple sets of acoustic token HMMs trained on the same corpus.
%
We call the level of representation corresponding to a granularity configuration a layer in the discussion below.
%
Note that with more parameters, the Multigranular paradigm is computationally heavier than the Hierarchical Paradigm.

\subsection{Model Granularity Space for Multi-layered token Sets}\label{ssec:mult_par0}

\begin{figure}[t]
\centerline{\includegraphics[width=0.45\textwidth]{figure/icassp_2015-3.png}}
\caption{Model granularity space for acoustic token configurations}\label{fig:2dcube}
\end{figure}

Here each layer of acoustic token is defined by a set of temporal and phonetic granularity parameters.
%
Contrary to the mutually dependent two-layer structure (word-like and subword-like) in the Hierarchical Paradigm, different layers of tokens are discovered independently of each other in the Multigranular Paradigm.
%
The HMM training is similar to the Eqs. (\ref{eq:1}) to (\ref{eq:3}) in the Hierarchical Paradigm with the following differences.
%
In the initialization step, only the cluster ids of subword-like tokens in Fig. \ref{fig:WS} are kept and the word-like structure is discarded, and only stage (I) in Fig. \ref{fig:FP} is applied while stages (II) and (III) are omitted.
%
In other word, here $\theta=\theta^a$, while $\theta^x$ and $\theta^l$ (the lexicon and language model for word-like tokens) in the Hierarchical Paradigm in Section \ref{sec:hier_par} are not used in this paradigm.
%
The process of initialization in Eq. (\ref{eq:1}) followed by stage (I) in Fig. \ref{fig:FP} can be performed with many different HMM configurations $\psi$.


Each HMM configuration is characterized by two hyperparameters: the number of states $m$ in each acoustic token HMM, and the total number of distinct acoustic tokens $n$ during initialization, with $\psi=(m,n)$ used to represent the model configuration. 
%
The transcription of a signal decoded with these tokens can be considered as a temporal segmentation of the signal, so the HMM length (or number of states in each HMM) $m$ represents the temporal granularity. 
%
The set of all distinct acoustic tokens can be considered as a segmentation of the phonetic space, so the total number $n$ of distinct acoustic tokens represents the phonetic granularity. 
%
This gives a two-dimensional representation of the acoustic token configurations in terms of temporal and phonetic granularities as in Fig. \ref{fig:2dcube}. 
%
Any point $\psi=(m,n)$ in this two-dimensional space in Fig. \ref{fig:2dcube} corresponds to an acoustic token configuration. 
%
Note that there can be a third dimension, the acoustic granularity which is the number of Gaussians in each HMM state, but the effect of that dimension will be shown to be negligible in the experiments below, thus we simply set the number of Gaussians in each state to be 4 unless explicitly stated. 
%
Although the selection of the hyperparameters can be arbitrary in this two-dimensional space in principle, here we simply select $M$ temporal granularities and $N$ phonetic granularities, forming a two-dimensional array of $M \times N$ hyperparameter sets in the granularity space and $M \times N$ sets of acoustic tokens. We denote the collection of selected granularities to be $G$, as shown in Eq. (\ref{eq:G}).
\begin{equation}
G=\{(m_j, n_k)| 1\leq j \leq M, 1\leq k \leq N\} \label{eq:G}.
\end{equation}
Each label sequence $W$ in Eq. \ref{eq:1} to Eq. \ref{eq:3} is now replaced with $W^\psi$, and each acoustic token HMM set $\theta$ is now replaced with $\theta^\psi$  
%, $W=\{W^\psi | \psi \in G \}$ now refers to the collection of all $W^\psi$ 
as shown in Eq. (\ref{eq:mult_I}) to Eq. (\ref{eq:mult_M}).

\begin{eqnarray}
W^\psi_0 &=& \mbox{initialization}(X).      
\label{eq:mult_I} \\ 
\theta^\psi_{i} &=& \arg \max_{\substack{\theta^\psi}} P(X|\theta^\psi,W^\psi_{i-1}),   
\label{eq:mult_E} \\
W^\psi_i &=& \arg \max_{\substack{W^\psi}} P(X|\theta^\psi_i ,W^\psi).
\label{eq:mult_M}
\end{eqnarray}




==> section/unification_derive.tex <==
\section{Derivation of the bounds in Eq. \eqref{eq:card_hier}}\label{sec:hier_bound}
Model parameters for a token set under the Hierarchical Paradigm consist of two parts: %$\theta^a$ for the subword-like acoustic model, $\theta^l$ for the word-like token language model and $\theta^x$ for the word-like token lexicon.
%
%Here we ignore the word-like token language model $\theta^l$ and consider only the subword-like token acoustic model $\theta^a$ and word-like token lexicon $\theta^x$.
%
Let $\theta^{mn}_{uv}=\{\theta^{mn},\theta_{uv}\}$
%denote the parameters for a token set under the Hierarchical Paradigm with 
, or the subword-like token acoustic model $\theta^{mn}$ of granularity $(m,n)$ and the word-like token lexicon $\theta_{uv}$.
%
Because a word-like token is composed of one to several subword-like tokens, $u$ is a positive integer multiple of $m$.
%
%All HMMs in subword-token acoustic model $\theta^{mn}$ have $m$ states and there are $n$ distinct HMMs, which uses the same definition as the Multi-granular Paradigm.
%
Since the lexicon $\theta_{uv}$ limits the token sequence for any utterance to include only word-like tokens in the lexicon, the possible subword-like token sequences is a subset of the case with only the subword-like acoustic token model $\theta^{mn}$, hence we have
\begin{equation}
C(\theta^{mn}_{uv}) \leq C(\theta^{mn}). \label{eq:card_upper}
\end{equation}
%
On the other hand, with the Hierarchical Paradigm we represent the utterances as sequences of word-like tokens.
%
We have a total of $v$ allowed distinct word-like tokens and the maximum length of a word-like token is $u$.
%
%if we ignore the word-like structure of the lexicon, and treat every word-like token as a subword-like token we get an acoustic model with $v$ HMMs.
%
Since not all word-like tokens are composed of the same number of subword-like tokens in the lexicon, this set of $v$ word-like tokens would have mixed temporal granularity. This means the $v$ word-like tokens would have varying number of states with the longest having $u$ states.
%
The lower bound of the total number of token sequence representations for this situation is the case when all the $v$ word-like tokens in the lexicon have the same length of $u$ states.
%
This number is the same as a set of $v$ subword-like tokens each with $u$ states, or $\theta^{uv}$ for the Multi-granular Paradigm, therefore 
\begin{equation}
C(\theta^{uv}) \leq C(\theta^{mn}_{uv}). \label{eq:card_lower}
\end{equation}
%
%The number of possible outcomes of this acoustic model is going to be greater than an acoustic model with $v$ HMMs, with all the HMMs being composed of $u$ states (an acoustic model with granularity $\theta^{uv}$), so $C(\theta^{uv}) \leq C(\theta^{mn}_{uv})$.
%
By combining Eq. \eqref{eq:card_upper} and Eq. \eqref{eq:card_lower}, we can get an upper and a lower bound:
\begin{equation}
 C(\theta^{uv}) \leq C(\theta^{mn}_{uv}) \leq  C(\theta^{mn}). \label{eq:card_hierx}
\end{equation}
%

==> table/paradigm.tex <==
\begin{table*}[t]
\centering
\caption{Model-dependent minCnxe for different token sets under the two paradigms with varying granularities}
\label{tab:big_table}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
      &         & \multicolumn{2}{c|}{(A)}         & \multicolumn{2}{c|}{(B)}           & \multicolumn{2}{c|}{(C)}           &          \\ \cline{3-8}
Index & (m,n)   & \multicolumn{2}{c|}{Mult. Doc. Tokens} & \multicolumn{2}{c|}{Mult. Qer. Tokens} & \multicolumn{2}{c|}{Hier. Qer. Tokens} & (u,v)    \\ \cline{3-8}
      &         & Eq. \eqref{eq:dtw}       & Eq. \eqref{eq:dtw_p}        & Eq. \eqref{eq:dtw}       & Eq. \eqref{eq:dtw_p} & Eq. \eqref{eq:dtw}       & Eq. \eqref{eq:dtw_p}&          \\ \hline
(1)   & (3,100) & 0.8008        & 0.7838           & 0.7938         & 0.7856            & 0.8025         & 0.7921            & (6,582)  \\ \hline
(2)   & (3,200) & 0.7985        & 0.7842           & 0.8047         & 0.7847            & 0.8022         & 0.7905            & (6,878)  \\ \hline
(3)   & (5,100) & 0.7872        & 0.7651           & 0.7854         & 0.7804            & 0.7893         & 0.7822            & (10,379) \\ \hline
(4)   & (5,200) & 0.7929        & 0.7671           & 0.8010         & 0.7882            & 0.8036         & 0.7978            & (10,539) \\ \hline
(5)   & (7,100) & 0.7938        & 0.7672           & 0.7908         & 0.7814            & 0.7880         & 0.7841            & (14,320) \\ \hline
(6)   & (7,200) & 0.7833        & 0.7645           & 0.7966         & 0.7911            & 0.7950         & 0.7875            & (14,395) \\ \hline
(7)   & Average & 0.7826        & 0.7644           & 0.7828         & 0.7735            & 0.7923         & 0.7829            &  \\ \hline
\end{tabular}
\end{table*}

==> table/std_type.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[tbh]
\centering
\caption{Query Token}
\label{tab:std_qer_type}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
& (m, n) & (u, v) &T1 & T2 & T3 \\ \hline
\multirow{7}{*}{Mult.}
&(3, 100)    &-           &0.7860  &0.7987  &0.8139\\
&(3, 200)    &-           &0.7794  &0.8048  &0.8145\\
&(5, 100)    &-           &0.7862  &0.7984  &0.8062\\
&(5, 200)    &-           &0.7813  &0.7984  &0.8117\\
&(7, 100)    &-           &0.7795  &0.7990  &0.8075\\
&(7, 200)    &-           &0.7807  &0.8014  &0.8073\\
&average     &-           &0.7747  &0.7984  &0.8114\\ \hline
\multirow{7}{*}{Hier.}
&(3, 100)    &(6, 582)    &0.7819  &0.8051  &0.8139\\
&(3, 200)    &(6, 878)    &0.7819  &\textbf{0.7963}  &\textbf{0.8051}\\
&(5, 100)    &(10, 379)   &0.7817  &0.8013  &0.8131\\
&(5, 200)    &(10, 539)   &0.7786  &0.7966  &0.8103\\
&(7, 100)    &(14, 320)   &0.7822  &0.8046  &0.8090\\
&(7, 200)    &(14, 395)   &\textbf{0.7775}  &0.8079  &0.8065\\
&average     &-           &0.7774  &0.7960  &0.8026\\ \hline
\end{tabular}
\end{table}

\begin{table}[tbh]
\centering
\caption{Document Token}
\label{tab:std_doc_type}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
& (m, n) & (u, v) &T1 & T2 & T3 \\ \hline
\multirow{7}{*}{Multi.}
&(3, 100)    &-           &0.7820  &0.7967  &0.8128\\
&(3, 200)    &-           &0.7860  &0.7942  &0.8001\\
&(5, 100)    &-           &0.7722  &0.7886  &0.7732\\
&(5, 200)    &-           &0.7757  &0.7868  &0.7904\\
&(7, 100)    &-           &0.7727  &0.7908  &0.7885\\
&(7, 200)    &-           &0.7735  &\textbf{0.7797}  &0.7769\\
&average     &-           &0.7701  &0.7770  &0.7788\\ \hline
\multirow{7}{*}{Hier.}
&(3, 100)    &(6, 3338)   &0.7845  &0.8003  &0.7966\\
&(3, 200)    &(6, 8571)   &0.7840  &0.7987  &0.7953\\
&(5, 100)    &(10, 3904)  &\textbf{0.7713}  &0.7861  &\textbf{0.7613}\\
&(5, 200)    &(10, 9191)  &0.7780  &0.7895  &0.7729\\
&(7, 100)    &(14, 4119)  &0.7749  &0.7852  &0.7888\\
&(7, 200)    &(14, 8296)  &0.7736  &0.7798  &0.7920\\
&average     &-           &0.7706  &0.7805  &0.7915\\ \hline
\end{tabular}
\end{table}
